ChatGPT Asks, BLIP-2 Answers: Automatic Questioning Towards Enriched Visual Descriptions

Asking insightful questions is crucial for acquiring knowledge and expanding our understanding of the world. However, the importance of questioning has been largely overlooked in AI research, where models have been primarily developed to answer questions. With the recent advancements of large language models (LLMs) like ChatGPT, we discover their capability to ask high-quality questions when provided with a suitable prompt. This discovery presents a new opportunity to develop an automatic questioning system. In this paper, we introduce ChatCaptioner, a novel automatic-questioning method deployed in image captioning. Here, ChatGPT is prompted to ask a series of informative questions about images to BLIP-2, a strong vision question-answering model. By keeping acquiring new visual information from BLIP-2's answers, ChatCaptioner is able to generate more enriched image descriptions. We conduct human-subject evaluations on common image caption datasets such as COCO, Conceptual Caption, and WikiArt, and compare ChatCaptioner with BLIP-2 as well as ground truth. Our results demonstrate that ChatCaptioner's captions are significantly more informative, receiving three times as many votes from human evaluators for providing the most image information. Besides, ChatCaptioner identifies 53% more objects within the image than BLIP-2 alone measured by WordNet synset matching. Code is available at https://github.com/Vision-CAIR/ChatCaptioner

==> background.tex <==
\iffalse
\section{Backgrounds}

\subsection{InstructGPT and ChatGPT}
InstructGPT \cite{ouyang2022training} is a GPT-3 \cite{brown2020language} model that is trained to better align with human preferences and expectations. This is achieved through a three-stage training process. Firstly, GPT-3 is fine-tuned on a dataset that only contains examples of desired model behavior. Secondly, a reward model is trained to score the model's outputs based on human feedback. Finally, GPT-3 is further fine-tuned using the PPO \cite{schulman2017proximal} algorithm to maximize the reward function. 
Through InstructGPT's training process, ChatGPT \cite{openai2022chatgpt} has developed exceptional skills in tracking users' intent and keeping the conversation going smoothly.



\subsection{BLIP-2}
BLIP-2 \cite{li2023blip} is a state-of-the-art visual-language pretraining strategy that utilizes a lightweight Querying Transformer to convert visual features from a frozen pretrained ViT \cite{dosovitskiy2020image} model into a fixed set of semantically meaningful tokens. 
These tokens can be directly understood by a pretrained large language model (LLM).
By bridging the gap between the pretrained vision model and the pretrained LLM, this approach achieves impressive results across a variety of vision-language tasks. 
\fi
